Order Matters: Probabilistic Modeling of Node Sequence for Graph Generation

A graph generative model defines a distribution over graphs. One type of generative model is constructed by autoregressive neural networks, which sequentially add nodes and edges to generate a graph. However, the likelihood of a graph under the autoregressive model is intractable, as there are numerous sequences leading to the given graph; this makes maximum likelihood estimation challenging. Instead, in this work we derive the exact joint probability over the graph and the node ordering of the sequential process. From the joint, we approximately marginalize out the node orderings and compute a lower bound on the log-likelihood using variational inference. We train graph generative models by maximizing this bound, without using the ad-hoc node orderings of previous methods. Our experiments show that the log-likelihood bound is significantly tighter than the bound of previous schemes. Moreover, the models fitted with the proposed algorithm can generate high-quality graphs that match the structures of target graphs not seen during training. We have made our code publicly available at \hyperref[https://github.com/tufts-ml/graph-generation-vi]{https://github.com/tufts-ml/graph-generation-vi}.

==> author-response/rebuttal-backup-dont-use.tex <==
Thank reviewers for your feedback!

Evaluation with log-likelihoods: We should emphasize that our work focus on the autoregressive-based graph generation model, in which the log-likelihood is not well-defined. 

***Then we give responses to your comments below.
**Reviewer 4:
Q1. "are there important/practical applications?"  

A1. On the theory side, a good graph generation model can serve as a decoder in an variational autoencoder structure. In this case, the proposed model can improve representation learning of variational autoencoders for graphs. 

On the practical side, the model can be used to model graphs such as molecule graphs and enzyme graphs. The submission includes an enzyme dataset in experiments. 

We will discuss these applications in the next version.

Q2. So I don't understand how the proposed method opens the door for them?

A2. Our writing should have been clearer: we mean that this submission is the first to rigorously calculate the data log-likelihood of autogressive graph generation models (previous models and our model). We will make it clearer in next version.

Q4. In Eq (1), why the special termination symbol is conditioned on L? Similarly for Eq (2).
A4. The generative model needs a special action to terminate the generation process, just like the EOS in sentence generation. In the two equations, L or Gn represents the graph G itself, and the model needs to stop at this step to get G. 

Q5. In Eq (7), please clarify how to evaluate the joint distribution p(G, pi) for given G and pi, like in evaluating the ELBO in Eq (12)?
A5. In p(G, pi), G is an observed data point while pi is unobserved/unknown, so the evaluation of p(G, pi) can only depend on the marginal distribution p(G) = \sum_pi p(G, pi) is consists of two parts: 1) For the one with p(A), the calculation of p(A) is given in Eq (1), 

 p(G, pi) is consists of two parts:For the one with p(A), the calculation of p(A) is given in Eq (1), which can be treated as a conditional sequence generation process. In practice, it can be obtained directly from previous model, such as GraphRNN or GraphGEN. The factor 1/|A| is the number of the automorphism of graph G. This is to eliminate multiplicity caused from different \pi leading to the same A. This is the same with the one with p(G_1:n), except p(G_1:n) is from generation models based on graph sequence rather than A (such as DeepGMG), and multiplicity is the number of \pi leading to the same G_1:n. We have provided the detail calculation for this one in Eq(9,10,11).  


Q6. In the experiments, how do you evaluate the exact log-likelihood, for example in Figure 6?
A6. We evaluate the exact log-likelihood by enumerating all N! permutations given a graph. In general this is intractable when N is large. In Figure 6, we only estimate the exact log-likelihood for graphs with fewer than 10 nodes.

**Reviewer 5:
Q1. The writing is mostly clear, although the notation introducing the surjection from graph + ordering to adjacency matrix could probably be made a bit cleaner.
A1.

Q2. The weaknesses include the relative straightforwardness of the proposed method. Furthermore, it's a little difficult to appreciate log-likelihood as a metric, since the performance of the vanilla graph generative models is quite bad to begin with for some complicated graph families, so small changes in the likelihood are not extremely impactful.

A2. We want to again summarize our contribution here: 1) The definition of the log-likelihood in previous method is problematic, i.e., they ignore the graph automorphism problem when defining the join probability p(G,pi). Our method proposed to correct this issue (see section 2). 2) The previous models are trained either in uniform or canonical orderings. The former one have log-likelihood but perform bad, the latter one do not have log-likelihood but perform relatively well. Our method proposed the VI framework (section 3) to achieve both and obtain better performance and highly interpretable result (section 4). 3) The proposed method would have a good impact on the community, as now more and more autoregressive graph generative models are proposed and they all face the same problem. Our method is the general training framework that can apply to most of them. 

A2. The task for the model is to maximize the log-likelihood for graphs in the training set. The learned model can be treated as a distribution for graphs. We think the best way to test the quality of a distribution is the log-likelihood for data in the test set. And we are the first to provide this metric. Previous wokrs (GRAN) has indicated that naive graph statistics can not reflect the generated graphs well. We think it is beneficial to check the learned model from log-likelihood and the quality of generated graphs.

Q3. The fact that the variance is so low is quite surprising; does a heuristic look at the learned ordering distribution inform why? Indeed, without a loss term regularizing the posterior from collapsing, does it gravitate towards a single canonical ordering regardless (or a mixture of several equivalent orderings to respect the symmetry argument in Figure 1)?

No. From our observation, nodes share a relative fair probability to be selected as the first step, because GNN only captures local dependency. With different start point, the whole sequence be very different. Though the whole sequence may has some preferences (the next node tends to has edges connected to selected nodes, for example), it is hard to converge to a small set of sequence.

Yes. From Figure 7, we observe that the sampled sequence is limited to a set of orderings.


**Reviewer 7:
Incorporating node ordering to infer parameters of a graph generative model is an interesting problem and the proposed technique shows promising results with a non-trivial experimental set up. Although more details could be provided about the experiments and the assumptions for the estimation as I detail in the next paragraph, the overall structure of the paper is well organized.

Q1. Some points need some additional details. The paper assumption of the sequential graph generation implies that only one node or its orbit (and corresponding edges) at a time. This means that the node permutations are highly dependent on the initialization conditions. How this conditions affect the node permutation counting? There are cyclic dependencies depending on whether the initial nodes are high-degree or low-degree nodes. What can be done in these situations? It seems to me that higher-order dependencies may affect the performance of the technique. 
A1.

Q2. Finally, in the experimental section the paper mentions that default hyperparameters were used to train the baselines. How does this choice affect the comparison. Namely, what are the default hyperparameters used and can a different configuration lead to smaller differences?
A2. The default hyperparameters were used to train both the baselines (uniform orderings/canonical orderings) and our method (VI orderings), i.e., we keep the architecture of the generative models to be consistent so that only the orderings will be the only factor that determines the generative quality. The hyperparameters we explore is about the architectures of the posterior distribution. We explore 3 kinds of architectures (GCN, GAT, APPNP) with different hyperparameters, and 2 kinds of distribution (proposed orderings in one shot or sequentially). We will make it clearer in the latest (next?) version.


**Reviewer 8:
Q1. results show an improvement with respect to uniform sampling for the same methods. This could be expected, as the proposal is an improvement to uniform sampling.
A1. Our proposal aims to improve to not only uniform sampling but several canonical sampling orders (BFS, DFS, etc). Our method has outperformed the models trained under uniform and canonical orderings in terms of likelihood, visualization and graph characteristics. 

Q2. However, classical algorithms, such as Chung Lu, BTER, mKPGM, ERGM, SBM, etc. can replicate networks with millions of nodes with interpretable models. It is surprising, that current models based on GNN are not even compared against these methods, and instead, they compare against Erdos-Renyi, a very simple algorithm to generate graphs.
A2. GraphRNN report that their proposed method outperforms 4 classical algorithms (Erdos-Renyi,  Barabasi-Albert, mKPGM, SBM) on 4 datasets. So it has become a strong baseline for many deep graph generative models to compare with. Besides, current deep generative model doesn't necessarily base on GNN, methods related to RNN, VAE, GAN, RL are also very common. In our work, we focus on the deep generative models that rely on the RNN-like architectures and construct a posterior based on GNN.

It is true that in terms of the scalability, the current deep generative model is not comparable to the classical methods. ()

A2. In GraphRNN, they compare 4 classical algorithms including Kronecker, MMSB. The result shows that there is a huge advantage by using deep neural network. Actually, GranRNN or Graphgen model doesn't utilize GNNs for graph generation, though the task targeting on graph.  After transferring the generation process into a sequence of decisions, they both use LSTM to maximize the log-likelihood. But DeepGMG model indeed utilize GNN to get node representations in the graph. Traditional algorithms mainly generate graphs based on some graph statistics. For example, ERGM mainly focuses on edge count and the number of triangles combined with MCMC. The Barabasi-Albert model is carefully designed to capture the ´scale-free nature of empirical degree distributions. These algorithms fail to capture many other aspects of graphs, and complex structural dependencies. There are many previous works (GraphRNN, Graphgen, GRAN...)  indicating the limitations of these classical algorighms. 

% The goal of our work is trying to improve the deeplearning based models through VI. We will add more discussion in the related work and also experiments part to for classical algorithms.


Q3. Another important flaw is the evaluation process. Part of the evaluation is based on visual examples of the generated graphs (Figure 3). Instead, use local and global network characteristics. For example, you can compare the distribution for the degree, clustering, and geodesic distance. This is much more informative than current results. 
A3. We provide graph characteristics in Table 2. We adopt 3 structural evaluations: (1) node degree distribution, (2) clustering coefficient distribution of nodes, and (3) orbit count distribution, which measures the number of all orbits with 4 nodes. The result shows that the model can better fit graph structure characteristics with our algorithm. As a generative model, we think the best metric is log-likehood, provided in Table 1. The reason is that the graph characteristics do not necessarily reflect the graph property. One good example is that in Community-small + graphRNN, the model trained with uniform sampling also exhibit a small distance between ground-truth distribution and generative distribution. However, from the  graph visualization (Figure 3), we can see that it totally fails to generate a community structure.


Q4. Please include the training process in the paper. I think that is very relevant for your paper, instead of, for example, the visualization comparison of the sampled networks.
A4. Thanks for your suggestion. A sketch VI training process for graphRNN/graphGEN is in the appendix(A.2). We will provide a more detailed version in the latest version.

Thanks for the advice! We include the training process in the appendix(A.2). And we are planning to move it to the paper.

Q5. Can you apply this model to larger models?
A5. Yes. Our proposed framework are designed for all autoregressive graph generative models. (not sure is ask for larger model or larger graph)

Q6. Can the generative process model global characteristics such as cluster coefficient and geodesic distance distribution?
A6. (should merge to Q3) Yes. We provide cluster distributions in Table 2.



==> tables/labeled_graph_quality.tex <==
\begin{tabular}{lclcccclcccclcccc}
    \hline
        &&  \multicolumn{4}{c}{Lung} && \multicolumn{4}{c}{Yeast}&& \multicolumn{4}{c}{Cora}\\
    \cline{3-6}  \cline{8-11}\cline{13-16}
         && Deg. &  Clus. & Orbit  & Label && Deg. &  Clus. & Orbit& Label && Deg. &  Clus. & Orbit& Label \\
    \hline
        \multirow{3}{*}{GraphRNN}
        & bfs & 0.103 & 0.301& 0.043 &0.193 && 0.512 & 0.153 & 0.026 & 0.310 && 1.125 & 1.002 & 0.427 & 0.085\\
        & uniform  & 1.213 &  \textbf{0.002} &  0.081& 0.104 && 0.746 & 0.351 & 0.070 & 0.081 &&0.188 & 0.206 & 0.200 & \textbf{0.014}\\
        & Ours & \textbf{0.074} & 0.060 & \textbf{0.004} & \textbf{0.012} && \textbf{0.097} & \textbf{0.092} & \textbf{0.005} & \textbf{0.001} && \textbf{0.066} & \textbf{0.171} & \textbf{0.052} &0.314 \\
    \hline
        \multirow{2}{*}{GraphGEN}& dfs &0.049 &0.017 &0.0006 &\textbf{0.089} && 0.014&0.003 &0.000 &0.000 &&0.099 &0.167 &0.122 & 0.018 \\
        & Ours& \textbf{0.022} & \textbf{0.008}& \textbf{0.0004} &0.141 &&\textbf{0.012} &0.003 &0.000 &0.000 && \textbf{0.056} &\textbf{0.103} & \textbf{0.069} & \textbf{0.008} \\
    \hline
    \end{tabular}

==> tables/lowerbound_gaps.tex <==
%  \begin{tabular}{c|ccc}
%     \hline
%                     & marginal  & cr-lb     & vi-cr-elbo\\
%     \hline \hline
%         DGMG-q      & -124.7     & -124.8     & -131.8       \\
%         GraphRNN-q  & -68.1    & -68.1    & -75.2    \\
%         GraphGEN-q  &       -26.5    &  -26.6         &    -35.0       \\
%     \hline
%     \end{tabular}
